Reversible Jump Metropolis Light Transport using Inverse Mappings

We study Markov Chain Monte Carlo (MCMC) methods operating in primary sample space and their interactions with multiple sampling techniques. We observe that incorporating the sampling technique into the state of the Markov Chain, as done in Multiplexed Metropolis Light Transport (MMLT), impedes the ability of the chain to properly explore the path space, as transitions between sampling techniques lead to disruptive alterations of path samples. To address this issue, we reformulate Multiplexed MLT in the Reversible Jump MCMC framework (RJMCMC) and introduce inverse sampling techniques that turn light paths into the random numbers that would produce them. This allows us to formulate a novel perturbation that can locally transition between sampling techniques without changing the geometry of the path, and we derive the correct acceptance probability using RJMCMC. We investigate how to generalize this concept to non-invertible sampling techniques commonly found in practice, and introduce probabilistic inverses that extend our perturbation to cover most sampling methods found in light transport simulations. Our theory reconciles the inverses with RJMCMC yielding an unbiased algorithm, which we call Reversible Jump MLT (RJMLT). We verify the correctness of our implementation in canonical and practical scenarios and demonstrate improved temporal coherence, decrease in structured artifacts, and faster convergence on a wide variety of scenes.

==> background.tex <==
% !TEX root=paper.tex

\section{Background}
\label{sec:background}
This section introduces notation and definitions that are used in the remainder of the paper.
\cWAJ{This is redundant, but I added it because the transition seemed a bit hard.}

We are interested in solutions to the \emph{measurement equation}, which can be expressed as the integral
%
%
\begin{align}
    \Measurement_j = \int_\PathSpace \ReconFilter{j}(\xbar) \MContrib(\xbar) \dPath{\xbar} \punct{.} \label{eq:measurement-equation}
\end{align}
%
%
This equation computes the value of a measurement $\Measurement_j$ (usually, a pixel) in terms of an integral over all possible \emph{light paths}. The integrand is composed of the pixel reconstruction filter $\ReconFilter{j}(\xbar)$ and the contribution $\MContrib(\xbar)$ of light path $\xbar$. The domain of all such light paths is \emph{path space} $\PathSpace$. We can decompose $\PathSpace$ further into subdomains $\PathSpace^k$ that contain only light paths of a fixed length $k$, which together form $\PathSpace = \bigcup_{k=1}^\infty \PathSpace^k$. We summarize our notation in \tabref{tab:notation}.

\Paragraph{Monte Carlo Sampling.}
In traditional Monte Carlo methods, \equref{eq:measurement-equation} is approximated using the estimator
%
%
\begin{align}
    \Measurement_j \approx \frac{1}{N} \sum\limits_{i=1}^N \frac{\ReconFilter{j}\big(\xbar^{(i)}\big) \MContrib\big(\xbar^{(i)}\big)}{\pdf\big(\xbar^{(i)}\big)} \label{eq:mc-estimator}
\end{align}
%
%
with $N$ independent samples $\xbar^{(i)}$, where $\pdf(\xbar^{(i)})$ is the probability density of the $i$-th path sample.

\Paragraph{Primary Sample Space.}
We can express this sampling process more formally in terms of an abstract sampling scheme $\Pinv(\ubar)$, which takes a vector $\ubar$ of random numbers drawn uniformly, and generates a light path. The domain of these vectors forms \emph{primary sample space} $\PSSpace$. Similar to path space, we decompose this space over path lengths, such that $\PSSpace = \bigcup_{k=1}^\infty \PSSpace^k$ and $\PSSpace^k = [0, 1]^{\PSSpaceSize_k}$.
The dimensionality $\PSSpaceSize_k$ is chosen to be large enough such that all light paths of length $k$ can be sampled by $\Pinv$. This allows us to rewrite \equref{eq:mc-estimator} explicitly in terms of the sampling scheme, using the relation $\xbar^{(i)} = \Pinv\big(\ubar^{(i)}\big)$.

\Paragraph{Bidirectional Path Tracing.}
The choice of sampling scheme directly determines the variance of the estimator, and it is thus vital that $\pdf(\xbar^{(i)})$ is approximately proportional to the integrand to obtain an efficient integrator.
Many state-of-the art techniques build
on the family of samplers introduced in the \emph{bidirectional path tracing} (BDPT) framework, which constructs paths of length $k$ (i.e.\ with $k$ segments), using $k+2$ different sampling techniques $\Pinv_0(\ubar), \ldots, \Pinv_{k+1}(\ubar)$. For each sample, BDPT performs a weighted sum over the estimate computed from each sampling technique, where the $t$-th technique is weighted by the MIS weight $\misWeight_t$.

\Paragraph{Markov Chain Monte Carlo.}
MCMC sampling techniques 
generate correlated samples with a density that is exactly proportional to an arbitrary non-negative function $\StationaryDistribution(\CurrentState)$.
In most cases, they rely on the Metropolis-Hastings acceptance ratio:
given current state $\CurrentState$, a \emph{proposal} state $\NextState$ is drawn from a proposal distribution $\ProposalDistribution(\CurrentState \rightarrow \NextState)$. Next, with probability
%
\begin{align*}
    \AcceptanceP(\CurrentState \rightarrow \NextState) = \min \left\{1, \frac{\StationaryDistribution(\NextState) \ProposalDistribution(\NextState \rightarrow \CurrentState)}{\StationaryDistribution(\CurrentState) \ProposalDistribution(\CurrentState \rightarrow \NextState)}\right\}\!\punct{,}
\end{align*}
%
the proposal is accepted and becomes the next state of the Markov Chain; otherwise, it is rejected and the process repeats anew. Under relatively weak conditions on $\ProposalDistribution(\CurrentState \rightarrow \NextState)$, the distribution of Markov Chain states will converge to $\StationaryDistribution(\CurrentState)$.
%
%
In the context of Metropolis Light Transport, the Markov Chain operates on path space $\PathSpace$ and the target density $\StationaryDistribution$ is the path contribution $\MContrib(\xbar)$. A key issue is the choice of a proposal distribution: Although the Markov Chain will generally converge in the limit, a poor choice of proposals can either lead to low acceptance rates or excessive correlation between nearby states. Both reduce the \emph{mixing time}, i.e. the algorithm's ability to effectively explore the entire domain.

\Paragraph{Primary Sample Space MLT.}
PSSMLT leverages the existence of a sampling scheme $\Pinv(\ubar)$ for light paths, and operates the Markov Chain in primary sample space instead of path space. The target function $\MPSSTarget(\ubar)$ then becomes the composition of the path contribution and sampling scheme,
%
%
\begin{align}
    \MPSSTarget(\ubar) = (\MImportance \circ \Pinv)(\ubar)/\pdfPSS(\ubar) \punct{.}
\end{align}
%
%

PSSMLT is most often combined with BDPT~\cite{Kelemen:2002}, in which case
evaluating $\pdfPSS(\ubar)$ entails generating eye/camera subpaths and
determining the weighted contribution for all pairs of vertices. Unfortunately,
this sequence of steps is fairly expensive, and many of the vertex pairs will
generally contribute little to no energy.

\Paragraph{Multiplexed MLT.} MMLT~\cite{Hachisuka:2014} addresses this problem by making the availability of multiple sampling strategies transparent to the underlying Markov Chain. It does so by running separate Markov Chains for each path length $k$, in which the first dimension of primary sample space is used to select one of the $k+2$ techniques of BDPT. A perturbation in Multiplexed MLT may therefore change both the vector of random numbers, as well as which sampling technique is used to map that vector into a light path. Each Markov Chain uses the modified target function
%
%
\begin{align}
    \MPSSTarget_j(\ubar) = w_j(\ubar) (\MImportance \circ \Pinv_j)(\ubar)/\pdfPSS_j(\ubar) \punct{,}
\end{align}
%
%
which incorporates the MIS weight $w_j(\ubar)$ of the technique.
Thus, instead of evaluating all strategies all the time, this choice is adaptively made by the underlying Metropolis-Hastings iteration, allowing the method to focus the computation on successful sampling techniques that carry significant energy from the light sources to the camera.


==> previous-work.tex <==
% !TEX root=paper.tex
\section{Previous Work}
Current physically-based rendering algorithms all incorporate the concept of
numerical integration over sets of light paths, generally using a form of Monte
Carlo or Markov-Chain Monte Carlo sampling. Unbiased Monte Carlo rendering,
first pioneered with Kajiya's formulation of the Rendering
Equation~\shortcite{Kajiya:1986} and the path tracing algorithm, involves
averaging over independently sampled light paths to compute unbiased estimates
of the steady-state radiance. Bidirectional variants of path
tracing~\cite{Lafortune:1993,Lafortune:1996,Veach:1994} build on the reciprocal
nature of light transport to construct partial light paths from both camera and
light sources and connect them to yield large families of sampling strategies.
Each strategy importance samples different parts of the integrand, and the
resulting estimators are then combined into a joint estimator using some form
of \emph{multiple importance sampling} (MIS)~\cite{Veach:1995}.

MCMC Rendering algorithms such as MLT~\cite{Veach:1997} mark a significant
departure from classical Monte Carlo rendering. These methods generate
correlated sequences of light paths using local exploration, usually using
Metropolis-Hastings~\cite{Hastings:1970, Veach:1997} steps, or by simulating
Hamiltonian dynamics~\cite{Neal:2011, Li:2015}. 

\Paragraph{Path-Space MLT.} The original MLT algorithm by Veach and Guibas relies on a set of two mutation
strategies~(which change a path significantly) and three perturbation
strategies~(which change it only slightly). While mutations ensure that all
states are reachable, perturbations are the main tool by which the Markov Chain
locally explores the state space. Subsequent generalizations of these
strategies extend the perturbations to arbitrary chains of specular
interactions~\cite{Jakob:2013} and rough
materials~\cite{Kaplanyan:2014,Hanika:2015}. Other variations of MLT include
Energy Redistribution Path Tracing~\cite{Cline:2005}, which independently
simulates a large number of Markov Chains that are stratified in image space,
and Gradient-Domain Metropolis Light Transport~\cite{Lehtinen:2013}, which
estimates gradients and uses them to reconstruct the rendered image. A severe
problem with MLT and variations thereof is that admissible light paths lie on a
lower-dimensional subset of path space with non-Euclidean structure, which
tremendously complicates the design of mutations and perturbations. Existing
strategies only target specific physical effects, but modern scenes contain
many interactions types (e.g. scattering by fibers, subsurface scattering,
etc.) that may even occur simultaneously on a single light path.

\Paragraph{Primary Sample Space MLT.} PSSMLT~\cite{Kelemen:2002} takes a different approach that avoids these
problems: it is based on the observation that each iteration of a classical
Monte Carlo rendering algorithm (e.g. BDPT) consumes a limited number of random
variates and uses them to sample one or more light paths. These random variates
could also be generated ahead of time and considered as inputs of the path
tracer, which turns the remaining algorithm into a deterministic function.
PSSMLT then performs MCMC steps on a space of random variates, which admits
simple symmetric perturbation strategies due to its Euclidean structure. Any
reflectance model supported by the underlying rendering algorithm is
automatically handled by the resulting MCMC algorithm. The generality of this
approach has led to numerous applications, e.g. in the context of Photon
Tracing with MCMC sampling~\cite{Hachisuka:2011}, tempering techniques such as
Replica Exchange~\cite{Kitaoka:2009} and rendering algorithms steered by
arbitrary importance functions~\cite{Hoberock:2010,Gruson:2016}.
\emph{Multiplexed MLT} (MMLT)~\cite{Hachisuka:2014} improves the efficiency of
PSSMLT in conjunction with \emph{bidirectional path tracing} (BDPT) by allowing
the Markov Chain to adaptively focus computation on those bidirectional
sampling techniques that have a high contribution. This involves assigning a
special meaning to the first random number consumed by the algorithm, which we
review in Section~\ref{sec:background}.

\Paragraph{Reversible Jumps.} Our technique builds upon the Reversible Jump MCMC algorithm
(RJMCMC)~\cite{Green:1995}, which was originally developed in the area of
Bayesian Statistics. Bayesian applications of MCMC techniques involve sampling
from posterior distributions that take some form of evidence (e.g.
empirical observations) into account. RJMCMC addresses the case where
\emph{multiple} candidate models could describe a given set of observations,
and RJMCMC then extends the Metropolis-Hastings algorithm with mutations that
transition between these different models.
In our context, these models correspond to different bidirectional
sampling strategies that can construct the same path using a different number
of steps on the camera and light paths.

\Paragraph{Design space of MLT algorithms.} 
At a high level, we consider PSSMLT and MLT to be extremes in a space involving
a trade-off between the "opaqueness" of the underlying representation and the
design complexity of the resulting algorithm: the random number streams of
PSSMLT have no clear physical interpretation, but this also allows for PSSMLT's
concise and general perturbation strategy. In contrast, MLT operates on path
space, which is a direct encoding of the physical scattering process, but this
comes at a cost of significantly increased complexity. MMLT resembles PSSMLT,
though the special role of the first dimension of the random number stream
makes the representation slightly less opaque. The proposed RJMLT technique
lies squarely in between: by allowing an existing path to be turned back into
the random numbers that produce it, the distinction between primary sample
space and path space ceases to be significant. On the flipside, our method
requires the availability of inverse functions for many components of the
rendering system.

\begin{table}%
\caption{Table of notation}\label{tab:notation}%
    \begin{tabular}{ll}
    \toprule
        Symbol & Explanation \\
        \midrule
        $\PathSpace$ & Path Space \\
        $\PSSpace$ & Primary Sample Space \\
        $\PathSpace^k, \PSSpace^k$ & Spaces of paths of length $k$ \\
        $\PSSpaceSize_k$ & Size of $\PSSpace^k$ \\
        $\xbar$, $\ybar$ & Light paths \\
        $\ubar$, $\vbar$ & Random number vectors \\
        $\MContrib(\xbar)$ & Path contribution function \\
        $\pdf(\xbar)$ & PDF of sampling $\xbar$ \\
        $\MPSTarget(\xbar) = \MContrib(\xbar)/\pdf(\xbar)$ & PSSMLT importance function\\
        $\Pinv_i(\ubar)$ & $i$-th sampling technique of BDPT \\
        $\misWeightPSS_i(\ubar)$ & MIS weight of $i$-th technique \\
        $\pdfPSS_i(\ubar)$ & PDF of $i$-th technique \\
        $\MImportancePSS_i(\ubar)$ & $\MImportance(\Pinv_i(\ubar))$ \\
        $\MPSSTargetImportance_i(\ubar) = \misWeightPSS_i(\ubar) \MImportancePSS_i(\ubar)/\pdfPSS_i(\ubar)$ & MMLT importance function \\
        $\CurrentStateExPSS = (i, \ubar)$ & Extended state with explicit technique \\
        $\ProposalDistribution(\ubar \rightarrow \vbar)$ & Proposal density of $\vbar$ from state $\ubar$ \\
        $\AcceptanceP(\ubar \rightarrow \vbar)$ & Probability of accepting proposal $\vbar$ \\
        $\Jac{A}$ & Jacobian Matrix of function $A$ \\
\bottomrule%
    \end{tabular}
\end{table}

